Gen3DEval: Using vLLMs for Automatic Evaluation of Generated 3D Objects

Rapid advancements in text-to-3D generation require robust and scalable evaluation metrics that align closely with human judgment, a need unmet by current metrics such as PSNR and CLIP, which require ground-truth data or focus only on prompt fidelity. To address this, we introduce Gen3DEval, a novel evaluation framework that leverages vision large language models (vLLMs) specifically fine-tuned for 3D object quality assessment. Gen3DEval evaluates text fidelity, appearance, and surface quality by analyzing 3D surface normals, without requiring ground-truth comparisons, bridging the gap between automated metrics and user preferences. Compared to state-of-the-art task-agnostic models, Gen3DEval demonstrates superior performance in user-aligned evaluations, placing it as a comprehensive and accessible benchmark for future research on text-to-3D generation. The project page can be found here: \href{https://shalini-maiti.github.io/gen3deval.github.io/}{https://shalini-maiti.github.io/gen3deval.github.io/}.

==> figures/pretrain_data_distribution.tex <==
\begin{figure}
\vspace{-5cm}
\begin{center}
\includegraphics[width=1.\linewidth]{figures/pretrain_data_distribution_donut_idx.png}
\end{center}
\caption{\textbf{Data distribution for the pretraining dataset.} }
\vspace{-2mm}
\label{fig:pretraining_dataset_dist}
\end{figure}

==> figures/supp_imenc_comp_fig3.tex <==
\begin{figure*}
\vspace{-1.cm}
\begin{center}
\includegraphics[width=1.\linewidth]{figures/supp_imenc_comp3.pdf}
\end{center}
\vspace{-1.5cm}
\caption{\textbf{Qualitative result from ablation study on different input image embeddings.} This image shows an advantage of \shortmethod using CLIP combined with DinoV2 compared to  standalone CLIP embeddings.}

\label{fig:supp_imenc_comp3}
\end{figure*}

==> tables/method_ablations.tex <==
\begin{table*}
\centering
\begin{tabular}{lccccccc}
    &\multicolumn{2}{c}{Appearance} & \multicolumn{1}{c}{Surface} & \multicolumn{2}{c}{T-Fidelity}\\
    \cmidrule(lr){2-3} \cmidrule(lr){4-4} \cmidrule(lr){5-6}  
    & {Human} & {Synthetic} & {Synthetic} & {Human} & {Synthetic} & \\
    \midrule
    \multicolumn{5}{l}{\textbf{Image Encoders}} \\
     CLIP  & 0.87  & 0.991 & 1 & 0.74 & 1 & \\
     CLIP + Fit3D  & 0.84  & 1 & 1 & 0.64 & 1 &\\
     CLIP + DinoV2  & 0.9 & 1 & 1 & 0.75 & 0.74 & \\
     Fit3D  & 0.74 & 0.95  & 0.99 & 0.69 & 0.95 & \\
     DinoV2  & 0.8 & 1 & 1 & 0.65 & 0.9 & \\
    % \midrule 
    % \multicolumn{5}{l}{\textbf{Dataset Scaling}} \\
    %  25\% & 0.64 & 0.83 & 0.99 & 1 & 0.98 & \\
    %  50\% & 0.63 & 0.87 & 0.96 & 1 & 0.99 & \\
    %  75\% & 0.58 & 0.84 & 0.83 & 1 &  1 & \\
    \bottomrule
    \end{tabular}
\caption{We report accuracy for ablation studies on curated synthetic and human evaluation datasets. \label{tbl:method_ablations}}
\end{table*}





==> tables/pretrain_dataset_composition.tex <==
\begin{table*}
\begin{centering}
\renewcommand{\arraystretch}{1.4}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|lcc|}
\toprule 
Data Type & Description & Number of samples \tabularnewline
\midrule 
Single RGB & QA with a single view RGB image of the 3D asset from a representative camera view and their textual description.& 40,002 \tabularnewline
2-view RGB & QA with 2 multiview RGB images of the 3D asset that are in the combination of either front and back camera views or left and right camera views. & 40,002  \tabularnewline
4 multiview RGB & QA with 4 multiview RGB images of the 3D asset from 4 views of the asset, front, right, back, left. & 40,002 \tabularnewline
Single RGB image grid & QA with a single RGB image grid composed of the 4 views of the 3D asset, along with its textual description. & 11381 \tabularnewline
4 multiview surface normals & A with 4 multiview images rendering the surface normals images of the 3D asset from 4 views camera views,i.e, front, right, back, left.& TBD \tabularnewline
4 multiview depth renders & A with 4 multiview images rendering the depth information images of the 3D asset from 4 views camera views,i.e, front, right, back, left.& TBD \tabularnewline
\bottomrule
\end{tabular}%
}
\par\end{centering}
\caption{\textbf{Pre-training dataset composition} \label{tbl:pretrain_dataset_composition}}

\end{table*}

==> tables/sft_dataset_composition.tex <==
\begin{table*}
\begin{centering}
\renewcommand{\arraystretch}{1.4}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|lcc|}
\toprule 
Data Type & Description & Number of samples \tabularnewline
\midrule 
\tabularnewline
Human preference data & Pairwise asset comparison data collected from trials from a set of text to 3D generation models. The prompts used here are from~\cite{dreamfusion}, which contains 404 prompts in total. 
We curated this further by using only the data items where all the evaluators (3 in total) unanimously chose the same 3D asset to be better. We split this dataset at a prompt level and used 90 percent for the finetuning dataset.& TBD \tabularnewline

Synthetic RGB comparison & QA with 8 images, 4 views per 3D asset where one asset is from the high quality 3D asset and other is perturbed on different parameters, such as modified captions, 3D quality perturbations such as deleting vertices, smoothing of textures and generating assets with slightly modified captions. & TBD \tabularnewline
\bottomrule
\end{tabular}%
}
\par\end{centering}
\caption{\textbf{Finetuning dataset composition} \label{tbl:sft_dataset_composition}}

\end{table*}

